Towards Robust and Reliable Algorithmic Recourse

As predictive models are increasingly being deployed in high-stakes decision making (e.g., loan approvals), there has been growing interest in post hoc techniques which provide recourse to affected individuals. These techniques generate recourses under the assumption that the underlying predictive model does not change. However, in practice, models are often regularly updated for a variety of reasons (e.g., dataset shifts), thereby rendering previously prescribed recourses ineffective. To address this problem, we propose a novel framework, RObust Algorithmic Recourse (ROAR), that leverages adversarial training for finding recourses that are robust to model shifts. To the best of our knowledge, this work proposes the first solution to this critical problem. We also carry out detailed theoretical analysis which underscores the importance of constructing recourses that are robust to model shifts: 1) we derive a lower bound on the probability of invalidation of recourses generated by existing approaches which are not robust to model shifts. 2) we prove that the additional cost incurred due to the robust recourses output by our framework is bounded. Experimental evaluation on multiple synthetic and real-world datasets demonstrates the efficacy of the proposed framework and supports our theoretical findings.

==> sub_hist.tex <==
*HAVE 5K CHAR*

In our past submission, reviewers brought up three primary concerns. The first concern was that our experimental setup is too similar to that of \citet{rawal2020can}, but we note that this is by design -- and also now explicitly state this in Sections 1 and 2: \citet{rawal2020can} identified a critical problem with non-robustness of algorithmic recourses, and we propose and evaluate the first solution to this problem. We carry out rigorous theoretical and empirical analysis to demonstrate the necessity and efficacy of our solution. The second concern was an unfortunate misconception that the baseline AR-LIME (adaptation of AR to non-linear models using LIME) is something that we introduced in this paper. However, as we now clearly state in Sections 3.3 and 5.1, AR-LIME is not new to this work and was already introduced and utilized in previous works \cite{Ustun_2019, rawal2020beyond}. We just employ the same strategy in our work and consider ROAR-LIME (adaptation of our framework ROAR to non-linear models using LIME). Finally, there was a concern that our theoretical analysis employed a Gaussian assumption. In response, we substantially improved Theorem 2 to hold on any distribution requiring only that the mean is finite (therefore subsuming commonplace distributions like Gaussian, Bernoulli, Multinomial etc.) and discuss how Theorem 1 holds for other distributions (Bernoulli, Uniform, Categorical) in the Appendix. Beyond addressing the aforementioned issues, we have also expanded our empirical evaluation to include the ROAR-MINT method, a causal recourse method augmented with our robust formulation, ROAR, as detailed in Section 5. 
